xCHEM: SDR-Based Multi-Link Channel Emulator for Real-Time Hardware-in-the-Loop Digital-Twin

This paper presents xCHEM, a radio-frequency channel emulator that inserts programmable channels between physical radios using a single NI USRP X4xx software-defined radio. External channel models stream impulse responses to its field-programmable gate array without firmware changes or interruption of signal processing. A streaming datapath implements six independently configurable directional channels across four radio interfaces. Each channel uses a sparse finite impulse response filter whose memory-backed delays decouple delay span from multiplier resources. The real and complex variants support 32 and 16 nonzero taps, respectively, with a maximum delay of 16666.62 ns and 4.069 ns resolution. Coefficient scaling and arithmetic right shifts control attenuation. Hardware measurements show root-mean-square errors of 9.5 ps in delay over the full span and 0.11 dB in attenuation. Multipath delays are recovered within one sample. An FPGA coefficient engine produces tested Doppler shifts from +/-1 Hz to +/-1 MHz with mean frequency errors below 0.032 Hz relative to quantized commands after carrier-offset calibration; at 200 Hz, it reduces the measured near-carrier spur by 53.3 dB compared with 1 kHz host updates.

==> Figures/ran_srs_tdlb.tex <==
% RAN VI-D -- TDL-B at DS = 200 ns, recovered from the gNB's own SRS channel
% estimates. 19/23 taps, CFR rms 0.12 dB against theory.
%
% Data: data/ran_srs_tdlb_{cir,taps,ideal}.csv, written by
% scripts/export_srs_tdlb_csv.py, which reuses srs_multitap's analysis through
% srs_report's ParquetSource -- the same computation as LCHEM_1x1_report.pdf.
%
% The CIR is from a SINGLE SRS occasion. Averaging occasions smears a tap
% profile: aligning them by cross-correlation is ambiguous whenever the profile
% is near-periodic, and it once made 32 equal taps look like 4.
%
% Red stems are the taps the emulator REALISED; grey circles the ideal
% TR 38.901 profile. They differ because each delay is quantised to the
% 4.069 ns FIR grid via a 10 ns wire tick, so taps closer than that merge --
% hence 19 distinct delays out of the profile's 23. Merging is by POWER, which
% preserves the specified PDP.
\begin{tikzpicture}
  \begin{axis}[
    lchem wide,
    xlabel={Delay (ns)},
    ylabel={$|h|$ (dB)},
    xmin=-60, xmax=1160, ymin=-45, ymax=8,
    xtick={0,250,500,750,1000},
    ytick={-40,-30,-20,-10,0},
    enlarge x limits=false,
    lchem top legend,
  ]
    % measured CIR, one occasion
    \addplot[line width=0.6pt, no marks, color=lchemDL0]
      table[col sep=comma, x=delay_ns, y=cir_db] {data/ran_srs_tdlb_cir.csv};
      \addlegendentry{measured CIR}

    % realised taps: stems from the floor
    \addplot[ycomb, line width=0.7pt, no marks, color=lchemDL1, lchem stem legend]
      table[col sep=comma, x=delay_ns, y=amp_db] {data/ran_srs_tdlb_taps.csv};
      \addlegendentry{realised taps}

    % ideal TR 38.901 profile
    \addplot[only marks, mark=o, mark size=1.3pt, color=lchemTheory]
      table[col sep=comma, x=delay_ns, y=amp_db] {data/ran_srs_tdlb_ideal.csv};
      \addlegendentry{TR 38.901 ideal}
  \end{axis}
\end{tikzpicture}


==> Figures/ran_srs_twotap.tex <==
% RAN VI-D -- two-tap delay sweep to the emulator's delay-line limit, measured
% through SRS. Delay placement error against the realised tap delay.
%
% Data: data/ran_srs_twotap.csv (scripts/export_srs_twotap_csv.py), 43 captures
% from the twotap_coarse and twotap_fine campaigns, each de-embedded against
% the pass-through of its OWN campaign.
%
% |error| on a log axis rather than recovered-vs-realised: on a y=x plot every
% point sits on the diagonal and the sub-nanosecond placement -- the actual
% result -- is invisible. Values are floored at 0.01 ns.
%
% Only the CIR-peak estimator is plotted. The CSV also carries a CFR-ripple
% estimate, which is more precise below ~7500 ns but aliases about the comb-2
% Nyquist delay beyond it (returning 2*NYQ - tau). Showing that here would put
% a failure of the MEASUREMENT on the same axes as the emulator's accuracy,
% where a 1000 ns error next to the delay-line limit reads as the emulator
% breaking down at long delay -- the opposite of the result. The Nyquist
% ceiling is stated in the text instead, as the reason this estimator is used.
\begin{tikzpicture}
  \begin{axis}[
    lchem wide,
    xlabel={Realised tap delay (\si{\micro\second})},
    ylabel={$|$delay error$|$ (ns)},
    ymode=log,
    xmin=0, xmax=8600,
    % coordinates stay in ns (the limits and the CSV are in ns);
    % only the tick LABELS are rescaled to microseconds
    xtick={0,2000,4000,6000,8000},
    xticklabels={0,2,4,6,8}, ymin=0.008, ymax=1.6,
    ytick={0.01,0.1,1},
    yticklabels={$0.01$,$0.1$,$1$},
    enlarge x limits=false,
  ]
    % the three limits. The delay line (8329 ns) and the comb-2 SRS Nyquist
    % (8333 ns) coincide to 4 ns -- both follow from 245.76 MHz / 2048 =
    % 120 kHz = 2 x 60 kHz -- so they share one marker.
    \draw[red!70!black, dashed, line width=0.6pt]
      (axis cs:2344,0.008) -- (axis cs:2344,1.6);
    \node[font=\scriptsize, color=red!70!black, rotate=90, anchor=south east]
      at (axis cs:2344,1.35) {cyclic prefix};
    \draw[green!35!black, dashed, line width=0.6pt]
      (axis cs:8331,0.008) -- (axis cs:8331,1.6);
    \node[font=\scriptsize, color=green!35!black, rotate=90, anchor=south east]
      at (axis cs:8331,1.35) {delay line};

    % the 1 ns line: every point sits below it
    \draw[lchemTheory, dashed, line width=0.6pt]
      (axis cs:90,1) -- (axis cs:8600,1);
    \node[font=\scriptsize, color=lchemTheory, anchor=north west]
      at (axis cs:120,0.93) {\SI{1}{\nano\second}};

    \addplot[only marks, mark=*, mark size=1.3pt, color=lchemDL0]
      table[col sep=comma, x=tau_ns, y=abserr_cir_ns] {data/ran_srs_twotap.csv};
  \end{axis}
\end{tikzpicture}

